PET: An Annotated Dataset for Process Extraction from Natural Language Text

Process extraction from text is an important task of process discovery, for which various approaches have been developed in recent years. However, in contrast to other information extraction tasks, there is a lack of gold-standard corpora of business process descriptions that are carefully annotated with all the entities and relationships of interest. Due to this, it is currently hard to compare the results obtained by extraction approaches in an objective manner, whereas the lack of annotated texts also prevents the application of data-driven information extraction methodologies, typical of the natural language processing field. Therefore, to bridge this gap, we present the PET dataset, a first corpus of business process descriptions annotated with activities, gateways, actors, and flow information. We present our new resource, including a variety of baselines to benchmark the difficulty and challenges of business process extraction from text. PET can be accessed via huggingface.co/datasets/patriziobellan/PET

==> sections/agreementtablesentitytogether.tex <==
\begin{table}
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB A
\subcaption{Process Elements}
\label{tbl:annotationagreementelements}
\subcaption{subtable no. 1}
\end{subtable}%
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB B
\subcaption{Relations}
\label{tbl:annotationagreementrelations}
\end{subtable}
\caption{Annotators Agreements}
\end{table}

==> sections/baselinesresultsB2B3.tex <==
\scalebox{0.7}{
\begin{tabular}{|l|c|c|c||c|c|c|}
\hline
\multicolumn{3}{c||}{\textbf{Baseline 2}} & 
\multicolumn{3}{c|}{\textbf{Baseline 3}} \\
& Precision & Recall &F1 & Precision & Recall & F1 \\
\hline
Sequence Flow & 1.000 & 0.787 &	0.881 & 1.000 & 0.370 &	0.540 \\
\hline
Uses & 1.000 & 0.891 & 0.942 & 1.000 & 0.488 & 0.656 \\
\hline
Actor Performer	& 0.992 & 0.808 & 0.891 & 0.994 & 0.534 & 0.694 \\
\hline
Actor Recipient	& 0.993 & 0.817 & 0.896 & 1.000 & 0.476 & 0.645	\\
\hline
Further Specification & 1.000 & 0.828 & 0.906 & 0.875 & 0.109 & 0.194 \\
\hline
Same Gateway & 0.973 & 0.837 & 0.900 & 0.897 & 0.605 & 0.722	\\
\hline
Overall	& 0.997 & 0.825 & 0.903 & 0.994 & 0.438 & 0.608 \\
\hline
\end{tabular}
}

==> sections/entitystatistics.tex <==



==> sections/problembackground.tex <==
\section{Problem Background}
\label{sec:problem-background}
The extraction of process models from documents is a complex task, since the analysis of the natural language description of a process has to take care of the multiple linguistics levels (syntactical, semantics, and pragmatics) and to mitigate linguistic phenomena such as syntactic leeway, simultaneously.
Moreover, it has to handle the multiple possible interpretations (in terms of process behavior) that can be inferred from the same text, because the same semantic can be conveyed in multiple ways, maybe not always equivalent.
For example, there are different ways to represent, in a process model, a repeated event or activity, but it may be the case that only one of these possible interpretations is the correct one to represent in the formal model.

\begin{figure*}[ht] 
\centering
\includegraphics[scale=0.8]{taskexample.png}
\caption[An example of a text-to-model mapping]{Example of a text-to-model mapping \cite{van2017comparing} in which the meaningful activities described in the process description (on the left) are mapped to the process model diagram (on the right). Two interesting aspects are worthy to note. First, not all the sentences correspond to a process model element. Second the logical succession described in the text differs to the written sentences' order (as for example happens with sentences 4 and 5).}
\label{img:exampletexttomodel}
\end{figure*}

Figure~\ref{img:exampletexttomodel} presents an example of the process extraction task. The gray shadow boxes link each process description sentence on the left of the figure that describes a process element to its corresponding process element in the process diagram, represented in BPMN, on the right part of the figure.
Here, the ninth sentence can also be represented in different ways than the one reported in the diagram.
It is possible to represent the same semantic, for example, adopting a sub-process element (in case we need to re-use this part of the diagram somewhere else), or as a multi-instance activity (either parallel or sequential).
    
In general, the first task to perform when analyzing a process description regards filtering \textit{uninformative sentences} of the process description out, because not all the sentences represent a process elements.
Then, Actions, Actors, Events, Gateways, Artifacts, and various types of process flows can be extracted.
However, not only each sentence can describe multiple process elements, but also each word can have multiple meanings.
To determine the correct intended meaning and to map it into the corresponding process element implies considering these two aspect at once.
Finally, process elements discovered have to be logically organized following the semantic conveyed in the process description.
So, defining the \textit{logical succession of process model elements} is another challenge to tackle.

Figure~\ref{img:texttomodelabstractview} shows an abstract level of the \pet~task that is conceptualized as an algorithmic function \textit{f} that aims to ``map'' a natural language process description into its process model.
In the figure the process description is represented with the blue document icon on the left, and the process model generated from the function \textit{f}, represented on the right as a BPMN diagram.

\begin{figure*}[ht]  % {img:text-to-model-abstract-view}
\centering
\includegraphics[scale=0.9]{text-to-model.png}
\caption[Text-to-model approach, an abstract view]{The figure shows an abstraction of the algorithmic function \textit{f} that maps a natural language process description (represented with the blue document icon) to its formal representation, the process model diagram (displayed on the right part of the figure).}
\label{img:texttomodelabstractview}
\end{figure*}

% To solve the problem of \pet~one could rely on three approaches.
% The first solution aims to \textit{directly map} a process description into its process model representation.
% Artificial Neural Networks are the only set of statistical techniques that can perform this transformation.
% However, the huge quantity of data required to learn a model, and the small quantity of data available makes this strategy unfeasible.
% The second approach would be to extract a process model with a \textit{complex and ad-hoc tailored pipeline}.
% But, the advantage of a tailored transformation function could be a drawback when the function \textit{f} is applied into different contexts.
% The common solution found in the literature, presented in Figure~\ref{img:text-to-model-two-steps-transformation-approach}, performs a \textit{two-steps transformation approach with intermediate representation} (also called \textit{World Model}) to extract and create a process model.
% In the figure, the process document is represented with the black document icon on the left. 
% Here, the algorithmic function is considered as a \textit{compound} function.
% Firstly, \textit{$f_{a}$} extracts process elements from text and populates the intermediate representation (world model), represented with the world icon at the center of the figure, the process elements extracted.
% Then, \textit{$f_{b}$} generates the corresponding process model diagram, presented as a BPMN diagram in the right part of the figure, from the the world model.

% \begin{figure}[htbp] % {img:text-to-model-two-steps-transformation-approach}
% \centering
% \includegraphics[scale=0.5]{text-to-model-extend.png}    
% \caption[Two steps transformation approach]{The figure presents an abstract view of the \textit{Two steps transformation approach with intermediate representation}. The first function (\textit{$f_{a}$} extracts process elements form a text and memorize them into a process model (also called word model). The second function (\textit{$f_{b}$}) draws the process diagram starting from the data of the intermediate representation.}
% \label{img:text-to-model-two-steps-transformation-approach}
% \end{figure}

==> sections/togetherElementAgreementB1.tex <==
\begin{table}
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB A
\subcaption{Process Elements}
\label{tbl:annotationagreementelements}
\subcaption{subtable no. 1}
\end{subtable}%
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB B
\subcaption{Relations}
\label{tbl:annotationagreementrelations}
\end{subtable}
\caption{Annotators Agreements}
\end{table}

==> sections/together_scheleton.tex <==
\begin{table}
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB A
\subcaption{Process Elements}
\label{tbl:annotationagreementelements}
\subcaption{subtable no. 1}
\end{subtable}%
\begin{subtable}[c]{0.5\textwidth}
\centering
%TAB B
\subcaption{Relations}
\label{tbl:annotationagreementrelations}
\end{subtable}
\caption{Annotators Agreements}
\end{table}
